S$^2$AC: Energy-Based Reinforcement Learning with Stein Soft Actor Critic

Learning expressive stochastic policies instead of deterministic ones has been proposed to achieve better stability, sample complexity, and robustness. Notably, in Maximum Entropy Reinforcement Learning (MaxEnt RL), the policy is modeled as an expressive Energy-Based Model (EBM) over the Q-values. However, this formulation requires the estimation of the entropy of such EBMs, which is an open problem. To address this, previous MaxEnt RL methods either implicitly estimate the entropy, resulting in high computational complexity and variance (SQL), or follow a variational inference procedure that fits simplified actor distributions (e.g., Gaussian) for tractability (SAC). We propose Stein Soft Actor-Critic (S$^2$AC), a MaxEnt RL algorithm that learns expressive policies without compromising efficiency. Specifically, S$^2$AC uses parameterized Stein Variational Gradient Descent (SVGD) as the underlying policy. We derive a closed-form expression of the entropy of such policies. Our formula is computationally efficient and only depends on first-order derivatives and vector products. Empirical results show that S$^2$AC yields more optimal solutions to the MaxEnt objective than SQL and SAC in the multi-goal environment, and outperforms SAC and SQL on the MuJoCo benchmark. Our code is available at: https://github.com/SafaMessaoud/S2AC-Energy-Based-RL-with-Stein-Soft-Actor-Critic

==> Appendices/proof_hmc_likelihood.tex <==

\subsection{Proof of Theorem~\ref{thm:hmc_entropy}}
\label{sec:hmc_entropy}

\begin{theorem*}
Under condition: the first order derivative $\nabla_{a^l} Q(s,a^l)$ is Lipschitz continuous along each dimension with a Lipschitz constant $\ll 2/\epsilon^2$, \ie $||\nabla_{a^l}^2 Q(s,a^l)||_{\infty}\ll \epsilon^2$, the closed-form of $\log q^T(a^T)$ of HMC sampler is 
\begin{equation*}\small
\log q^T(a^T) = \log q^0(a^0) - \sum_{l = 0}^{L-1} (\epsilon^2/2) \Tr \big(\nabla_{a^l}^2 Q(s,a^{l})\big) 
\end{equation*}
\end{theorem*}


% \begin{align*}
% \nabla_{a^l} a^{l+1}&= \nabla_{a^l} a^{l} + \epsilon \nabla_{a^l} v^{l+1/2} \\
% &= I + \epsilon \nabla_{a^l} v^{l} + \epsilon(\epsilon/2) \nabla_{a^l}^2 Q(s,a^l)\\ 
% & = I + (\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^l)
% \end{align*}
% Here $\nabla_{a^l} v^{l}=0$ because $v^{l}$ and $a^{l}$ are independent by definition of HMC.

\begin{proof}
%In this proof, we omit the state $s$ in $Q(s,a^{l})$ for simplicity of notation.
Using the first two half steps of updates in Eq.\eqref{eq:hmc_update}, we have
\begin{align*}
&a^{l+1}\\
=& a^{l} + \epsilon v^{l+1/2} \\
=& a^{l} + \epsilon \left(v^l + (\epsilon/2) \nabla_{a^l} Q(s,a^l) \right)
%&= a^{l} + \epsilon v^l + (\epsilon^2/2) \nabla_{a^l} Q(s,a^l)
\end{align*}
Write it in the form of $F(a)=a+\epsilon h(a)$, we have $h(a)=v^l + (\epsilon/2) \nabla_{a^l} Q(s,a^l)$. Therefore, 
\begin{align*}
& \nabla_{a^l}h(a) \\
= & \nabla_{a^l} (v^l + (\epsilon/2)\nabla_{a^l} Q(s,a^l))\\
= & (\epsilon/2)\nabla_{a^l}^2 Q(s,a^l)
\end{align*}
Here $\nabla_{a^l} v^{l}=0$ because $v^{l}$ and $a^{l}$ are independent by definition of HMC. According to Proposition~\ref{prop:hmc_invertibility}, the HMC update function $F(a)$ is invertible. When the first order derivative $\nabla_{a^l} Q(s,a^l)$ is Lipschitz continuous along each dimension with a Lipschitz constant no larger than $ 2/\epsilon^2$, \ie $||\nabla_{a^l}^2 Q(s,a^l)||_{\infty}\ll \epsilon^2$, then it satisfies the condition 
\begin{align*}
\epsilon ||\nabla_{a^l} h(a^l)||_{\infty} = \epsilon ||(\epsilon/2)\nabla_{a^l}^2 Q(s,a^l)||_{\infty} \ll 1 
\end{align*}

Hence Theorem~\ref{thm:generic_entropy} holds for the HMC dynamics. Substituting the above expression of $h(a^l)$ to Eq.\eqref{eq:generic_entropy}, we have 
\begin{align*}
\log q^{L}(a^L)
%= & \log q^0(a^0) - \sum_{l = 0}^{L-1} \Tr \left( \nabla_{a^l} (v^l + (\epsilon/2)\nabla_{a^l} Q(s,a^l)) \right)\\
%\Tr \big((\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^{l})\big) \\
= \log q^0(a^0) - \sum_{l = 0}^{L-1} (\epsilon^2/2) \Tr \big(\nabla_{a^l}^2 Q(s,a^{l})\big) 
\end{align*}
Unfortunately, this involves the computation of the Hessian of $Q(s,a^l)$, which is computationally more costly than that of SVGD-based sampler. Thus we choose to use the latter as the underlying sampler for our action sampling component.
\end{proof}

%\hp{Will put the first order derivative Lipschitz continuity condition in Theorem~\ref{thm:hmc_entropy}. Similarly, we can make assumptions of such to make sure $I + (\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^t)$ is invertible (positive definite). This is useful: https://math.stackexchange.com/questions/1742753/lipschitz-implies-bounded-gradient}
% \begin{align*}
% \log q^{T}(a^T) &= \log q^0(a^0) - \sum_{t = 0}^{L-1} \log \Big| \det \nabla_{a^{l}} a^{l+1}  \Big| \\
%                 &= \log q^0(a^0) - \sum_{t = 0}^{L-1} \log \Big| \det \big(I +(\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^{t-1})\big) \Big|
% \end{align*}
% According Jacobi's formula, given an invertible matrix $A$,
% \begin{align*}
% \log (\det A) = \Tr(\log A) \approx \Tr(A-I)
% \end{align*}
% Here the approximation holds when $\|A-I\|_{\infty}\ll 1$.

% Let $A=I + (\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^t)$, then $\|A-I\|=(\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^t)$, the above condition holds as long as the first order derivative $\nabla_{a^l} Q(s,a^t)$ is Lipschitz continuous along each dimension with a Lipschitz constant $L\ll 2/\epsilon^2$

% Hence, we have
% \begin{align*}
% \log q^{T}(a^T) = \log q^0(a^0) - \sum_{t = 1}^{T} \Tr \big((\epsilon^2/2) \nabla_{a^l}^2 Q(s,a^{t-1})\big) 
% \end{align*}

==> Appendices/proof_ld_likelihood.tex <==
\textbf{Closed for expression of Langevin dynamics Induced Policy}
Langevin dynamic update rule: $a^{l+1}_{i} \leftarrow a^{l}_{i} + \epsilon, g(a^{l}_{i})$, with 

\begin{equation}
g(a^{l}) = \epsilon \nabla_{a^{l}} Q(a^{l},s) + \eta 
\end{equation}

We follow a similar procedure as above and obtain:

\begin{eqnarray*}
\log p(a^{L}|s)&=&\log p(a^{0}|s)-\sum_{l=0}^{L-1}\log \Big|\det \frac{a^{l+1}}{a^{l}} \Big|\\
&=&\log p(a^{0}|s)-\sum_{l=1}^{L-1}\log \Big|\det \Big(I + \epsilon \nabla_{a^{l}} g(a^{l})\Big) \Big|\\
&\approx& \log p(a^{0}|s)-\sum_{l=0}^{L-1}\epsilon \, \text{tr} \Big(\nabla_{a^{l}} g(a^{l})\Big)\\
&=& \log p(a^{0}|s)-\sum_{l=0}^{L-1} \epsilon^{2} \text{tr} \left( \nabla_{a^{l}}^{2} Q(a^{l},s)\right) \\
\end{eqnarray*}

In case the Hessian is symmetric, we can actually compute the trace with just vector operations.

It's possible to compute a stochastic estimator of the trace using the Hutchinson trick: $tr(A)= \mathbb{E}_{z}[z^T A z]$. with $z$ being random variables satisfying $\mathbb{E}_{z}[zz^T]=I$, for instance $z$ can be radamacher randomvariables or be drawn from a normal distribution. 

\begin{equation}
\text{tr}(\nabla_{a^{l}}^{2} Q(a^{l},s)) = \mathbb{E}_{z}[z^T \nabla_{a^{l}}^{2} Q(a^{l},s)  z]= \mathbb{E}_{z}[z^T \nabla_{a^{l}}\left(\nabla_{a^{l}} Q(a^{l},s)^T  z \right)]
\end{equation}


==> Results/landmark_experiments.tex <==

Why is this important?
What's a landmark?

\textbf{Supervised learning vs RL}:  check background and motivation section in \cite{8187667}.

Supervised mehod are either computationally inefficient (\eg scanning based systems, end-to-end systems) or are difficult to train due to poor robustness to variations in the image anatomical range(\eg regression-based systems). 

RL finds a 3d trajectory in the image space starting from a random position leading to a landmark


RL solutions have been proven to be more scalable and precise \cite{8187667, ghesu2016artificial, alansary2019evaluating}. 

==> Results/mujoco_experiments.tex <==
\subsection{Mujoco Experiments}
\input{figures/Mujoco/mujoco_fig_param}
We evaluate STAC on four environments from the OpenAI gym benchmark suite \cite{brockman2016openai}, including Hopper-v2, Walker2d-v2, HalfCheetah-v2, and Ant-v2. As baselines, we use (1) DDPG \cite{gu2016q}, (2) PPO \cite{schulman2015trust}, (3) SQL \cite{haarnoja2017reinforcement}, (4) TD3 \cite{fujimoto2018addressing}, (5) IAF \cite{kingma2016improved}, and (6) SAC \cite{haarnoja2018soft}. The model hyperparameters are reported in Appendix \ref{appendix:jujoco}.
We train five different instances of each algorithm with different random seeds, with each performing one evaluation rollout every $1000$ environment steps. Results are shown in \Figref{fig:mujoco}. The solid curves correspond to the mean returns over the five trials and the shaded region represents the minimum and maximum. STAC is consistently better than SQL across all the environments and has comparable performance to SAC in two out of four environments.  
Run time results are reported in Table \ref{tab:run_time} of Appendix~\ref{appendix:jujoco}. 


%Some of these environments are characterized by narrow basins of effective hyperparameters which make it hard for sensitive algorithms on the hardest benchmarks leading to poor performance.

%SAC performs comparably to baseline methods on the easier tasks and outperforms them on the harder tasks both in terms of learning speed and final performance.

%SQL is slower than SAC and has a worst performance.


%\safa{
%\textbf{Limitations}: SVGD is not guaranteed to converge. Hence, we can't prove convergence of the entropy}




==> figures/Mujoco/mujoco_fig.tex <==
\begin{figure*}[htb]
\centering
\begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/Hopper_mujoco_wolegend.pdf}
    \caption{Hopper-v2}
    \label{fig:mujoco_hopper}
\end{subfigure} \hspace{2mm}
\begin{subfigure}{.23\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/Walker2d_mujoco_wolegend.pdf}
    \caption{Walker2d-v2}
    \label{fig:mujoco_walker2d}
\end{subfigure}
\begin{subfigure}{.23\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/HalfCheetah_mujoco_wolegend.pdf}
    \caption{HalfCheetah-v2}
    \label{fig:mujoco_halfcheetah}
\end{subfigure}
\begin{subfigure}{.23\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/Ant_mujoco.pdf}
    \caption{Ant-v2}
    \label{fig:mujoco_ant}
\end{subfigure}
\caption{Training curves on continuous control benchmarks. STAC performance is superior to SQL across all environments and comparable to SAC for Hopper-v2 and Ant-v2.}
\label{fig:mujoco}
\end{figure*}


==> figures/Mujoco/mujoco_fig_append.tex <==
\begin{figure*}[htb]
\vspace{-3mm}
\centering
\begin{subfigure}{0.4\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/ppo_Antfig_0517.pdf}
    \caption{Ant-v2}
    \label{fig:mujoco_ant}
\end{subfigure} \hspace{4mm}
\begin{subfigure}{.4\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Mujoco/ppo_Humanoidfig_0517.pdf}
    \caption{Humanoid-v2}
    \label{fig:mujoco_humanoid}
\end{subfigure}
% \begin{subfigure}{.23\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{figures/Mujoco/Ant_mujoco.pdf}
%     \caption{Ant-v2}
%     \label{fig:mujoco_ant}
% \end{subfigure}
\vspace{-2mm}
\caption{Additional training curves on the MuJoCo benchmarks. 
% In the legends, STAC corresponds to STAC($\phi,\theta$) and STACN corresponds to STAC($\phi$). 
STAC($\phi,\theta$) has superior performance than SQL and STAC($\phi$), and outperforms SAC on Humanoid-v2. }
\label{fig:mujoco_2env}
\end{figure*}


==> figures/ablation_study.tex <==

\subsection{Ablation Study}
To see how the different configurations of SVGD training affect the performance of STAC, we evaluate the following four hyperparameters: 1) Number of SVGD steps, 2) Number of SVGD particles, 3) SVGD learning rate, and 4) SVGD kernel variation (measured as standard deviation). For each hyperparameter, we observe three aspects of the SVGD training, namely 1) number of modes covered, 2) entropy, and 3) mean episode length (to reach the goals).

\textbf{Number of SVGD steps.} We varied the number of SVGD steps among $\{5, 10, 15\}$. When number of SVGD steps increases, more modes are covered in general (no clear trend?), entropy is lower, and it takes less mean episode length to reach the goals. 

\textbf{Number of SVGD particles.} We varied the number of SVGD particles among $\{5, 10, 15\}$. When number of SVGD particles increases, fewer modes are covered in general (no clear trend?), entropy is higher, and it takes more mean episode length to reach the goals. 

\textbf{SVGD learning rate.} We varied the SVGD learning rate among $\{0.01, 0.05, 0.1\}$. When SVGD learning rate increases, fewer modes are covered in general, entropy is higher (or close?), and it takes approximately the same mean episode length to reach the goals.

\textbf{SVGD kernel standard deviation.} We varied the SVGD kernel standard deviation among $\{0.1, 0.5, 1\}$. When SVGD kernel standard deviation increases, fewer modes are covered in general, entropy is higher, and it takes more mean episode length to reach the goals. We also evaluated a version where the kernel standard deviation is set adaptive (w.r.t.?). It turns out that the adaptive version covers all of the four modes quickly, achieves the lowerst entropy, and requires the least mean episode length to reach the goals. 
%\hp{reverse the legends of 0.1 and 0.5?} 


\begin{figure*}[htb]
\centering
\begin{subfigure}{.3\linewidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_steps_modes.png}
    \caption{Number of modes covered}
    \label{fig:ablation_steps_modes}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_steps_entropy.png}
    \caption{Entropy during the episode}
    \label{fig:ablation_steps_entropy}
\end{subfigure}
\begin{subfigure}{0.3\linewidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_steps_episode_len.png}
    \caption{Episode length}
    \label{fig:ablation_steps_episode_len}
\end{subfigure}
    \caption{Effect of SVGD steps. The x-axes for the three subfigures are respectively the number of training steps (or episodes?), time step at an episode, and number of training epochs. The x-axes are the same for the following three figures.}
    \label{fig:ablation_steps}
\end{figure*}


\begin{figure*}[htb]
\centering
\begin{subfigure}{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_particle_modes.png}
    \caption{Number of modes covered}
    \label{fig:ablation_particle_modes}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_particle_entropy.png}
    \caption{Entropy during the episode}
    \label{fig:ablation_particle_entropy}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_particle_episode_len.png}
    \caption{Episode length}
    \label{fig:ablation_particle_episode_len}
\end{subfigure}
    \caption{Effect of number of particles in SVGD.}
    \label{fig:ablation_particle}
\end{figure*}

\begin{figure*}[htb]
\centering
\begin{subfigure}{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_LR_modes.png}
    \caption{Number of modes covered}
    \label{fig:ablation_LR_modes}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_LR_entropy.png}
    \caption{Entropy during the episode}
    \label{fig:ablation_LR_entropy}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_LR_episode_len.png}
    \caption{Episode length}
    \label{fig:ablation_LR_episode_len}
\end{subfigure}
    \caption{Effect of SVGD learning rate.}
    \label{fig:ablation_LR}
\end{figure*}

\begin{figure*}[htb]
\centering
\begin{subfigure}{.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_sigma_modes.png}
    \caption{Number of modes covered}
    \label{fig:ablation_sigma_modes}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_sigma_entropy.png}
    \caption{Entropy during the episode}
    \label{fig:ablation_sigma_entropy}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\linewidth]{figures/ablation/ablation_sigma_episode_len.png}
    \caption{Episode length}
    \label{fig:ablation_sigma_episode_len}
\end{subfigure}
    \caption{Effect of the kernel standard deviation in SVGD.}
    \label{fig:ablation_sigma}
\end{figure*}



\textbf{Run-time.}



==> figures/multi-goal/entr_states.tex <==
\begin{figure} [t!]
\centering
 \includegraphics[width=0.6\linewidth]{figures/multi-goal/entr_states.pdf}
  \caption{Entropy values at different states. The entropy consistently decreases when approaching the goals. }
  \label{fig:multigoal_stac_qlandscape}
\end{figure}


==> figures/multi-goal/robustness.tex <==

\begin{figure*}[t!]
\centering

\begin{tabular}{ccccc}
& $\alpha=0.2$  &  $\alpha=1$  & $\alpha=10$ & $\alpha=20$ \\
\raisebox{\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{STAC}}  
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_stac_a02.pdf}
           & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_stac_a1.pdf}
           & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_stac_a10.pdf}
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_stac_a20.pdf}\\
\raisebox{\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{SAC}}   
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sac_a02.pdf}
           & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sac_a1.pdf}
             & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sac_a10.pdf  }
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sac_a20.pdf  }\\
\raisebox{\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{SQL}}   
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sql_a02.pdf  }
           & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sql_a1.pdf}
             & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sql_a10.pdf}
            & \includegraphics[width=.16\linewidth]{figures/new_figures/path_vis_sql_a20.pdf}
\end{tabular}
\caption{Visualization of the trajectories from policies learned with STAC, SAC and SQL at test time in the multi-goal environment. The state corresponds to the 2D position, \ie $x$ and $y$ coordinates. The initial position is the origin. The goals are depicted as red dots and the level curves show the reward. Unlike SAC and SQL, STAC consistently recovers the three modes and more frequently converges to $G_2$ and $G_3$ with increasing $\alpha$ (direction with the maximum entropy). \hp{Change caption} }
\label{fig:multi-goal-robustness}
\end{figure*}



%\begin{figure*}[htb]
%\centering
%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_stac_a02.pdf}
%    \caption{STAC, $\alpha=0.2$}
%    \label{fig:multi-goal_stac_a-0.2_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_stac_a1.pdf}
%    \caption{STAC, $\alpha=1$}
%    \label{fig:multi-goal_stac_a-1_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_stac_a10.pdf}
%    \caption{STAC, $\alpha=10$}
%    \label{fig:multi-goal_stac_a-10_robustness}
%\end{subfigure} 
%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_stac_a20.pdf}
%    \caption{STAC, $\alpha=20$}
%    \label{fig:multi-goal_stac_a-20_robustness}
%\end{subfigure}\\

%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sac_a02.pdf}
%    \caption{SAC, $\alpha=0.2$}
%    \label{fig:multi-goal_sac_a-0.2_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sac_a1.pdf}
%    \caption{SAC, $\alpha=1$}
%    \label{fig:multi-goal_sac_a-1_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sac_a10.pdf}
%    \caption{SAC, $\alpha=10$}
%    \label{fig:multi-goal_sac_a-10_robustness}
%\end{subfigure}
%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sac_a20.pdf}
%    \caption{SAC, $\alpha=20$}
%    \label{fig:multi-goal_sac_a-20_robustness}
%\end{subfigure}\\

%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sql_a02.pdf}
%    \caption{SQL, $\alpha=0.2$}
%    \label{fig:multi-goal_sac_a-0.2_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sql_a1.pdf}
%    \caption{SQL, $\alpha=1$}
%    \label{fig:multi-goal_sac_a-1_robustness}
%\end{subfigure}
%\begin{subfigure}{0.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sql_a10.pdf}
%    \caption{SQL, $\alpha=10$}
%    \label{fig:multi-goal_sac_a-10_robustness}
%\end{subfigure}
%\begin{subfigure}{.24\linewidth}
%    \includegraphics[width=\linewidth]{figures/new_figures/path_vis_sql_a20.pdf}
%    \caption{SQL, $\alpha=20$}
%    \label{fig:multi-goal_sac_a-20_robustness}
%\end{subfigure}
%    \caption{The trajectories of 20 different episodes of the same STAC/SAC policy at test time when an obstacle is placed.}
%    \label{fig:multi-goal_robustness}
%\end{figure*}


\begin{figure}[htb]
\centering
    \includegraphics[width=0.8\linewidth]{figures/new_figures/goals_obstacle_dist.pdf}
\caption{Probability of reaching a goal after hitting the obstacle for the two algorithms with different $\alpha$'s. \color{blue}[BILLEL: we got this by running the one trained agent 5 test runs with 5 different seeds where each test run has 20 episodes.]}
\label{fig:robustness_comparison}
\end{figure}


==> figures/teaser_new.tex <==
\begin{figure}
  \begin{center}
    \includegraphics[width=\textwidth]{figures/teaser2.pdf}
  \end{center}
  \caption{The three paradigms of MaxEnt RL -- STAC, SAC, and SQL. Solid lines indicate similarities while dashed lines indicate differences. When modeling the policy as a vanilla (non-parametrized) SVGD, STAC becomes a value-iteration algorithm like SQL. Different from SQL, STAC models the entropy explicitly. When using a parametrized SVGD as the policy, STAC becomes an actor-critic algorithm like SAC, with the major difference being the policy representation, \ie STAC can capture complex distributions using a sampler from EBMs while SAC uses a Gaussian for a policy.}
\end{figure}

==> figures/toy/kernel_variance.tex <==
\begin{figure} [t!]
\centering
 \includegraphics[width=0.8\linewidth]{figures/toy/kernel_distr2_.pdf}
  \caption{Estimated entropy for different SVGD kernel variances and number of particles for $p\!=\!\cN([-0.69,0.8],[[1.13, 0.82],[ 0.82,3.39]])$.\hp{check} The ground truth entropy is represented as the dashed green line.}
  \label{fig:kernel_variance}
\end{figure}


==> figures/toy/toy_g_fig.tex <==
\begin{figure} [t!]
\centering
 \includegraphics[width=1.0\linewidth]{figures/sld00.png}
  \caption{Entropy derived via Langevin dynamics  }
  \label{fig:ldynamics}
\end{figure}


\begin{figure} [ht]
\centering
 \includegraphics[width=1.0\linewidth]{figures/sld00.png}
  \caption{Entropy derived via Langevin dynamics  }
  \label{fig:ldynamics}
\end{figure}


==> figures/toy/toy_table_3.tex <==
\begin{figure}[H]
\centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{figures/toy/table3_a_.pdf}
        \caption{GMM distributions}
    \end{subfigure} \hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering         
        \includegraphics[width=0.85\linewidth]{figures/toy/table3_g_.pdf}
        \caption{Gaussian distributions}
    \end{subfigure}%
\vspace{-1mm}
\caption{Estimated entropy by SVGD w.r.t. number of steps ($\#s$) and particles ($\#p$).} %consistently increases with increasing number of modes of GMM distributions (top) and variance of Gaussian distributions (bottom), irrespective of the number of SVGD steps ($\#s$) and particles ($\#p$).
\label{fig:steps_particles_gmm_gaussian}
\vspace{-4mm}
\end{figure}



==> formulas.tex <==



\begin{equation}
    \pi(a|s) = \exp Q(s, a)/Z
\end{equation}

\begin{equation}
    l \in [1,L]
\end{equation}

\begin{equation}
    i \in [1,M]
\end{equation}


\begin{equation*}%\label{eq:change_of_variable}
\small
q^{l}(a^l) = q^{l-1}(a^{l-1}) \Big| \det\!\frac {\partial a^{l}} {\partial a^{l-1}}  \Big|^{-1}
\end{equation*}


\begin{equation*}
\epsilon \Delta f(a^{0}_{i})
\end{equation*}



\begin{equation*}
-3\sigma_{\theta}\!\leq\!a_{\theta}^{l}\!\leq\!3\sigma_{\theta}, \quad \forall l \in [1,L]
\end{equation*}
